Unsupervised Pre-trained Models from Healthy ADLs Improve Parkinson's Disease Classification of Gait Patterns

Application and use of deep learning algorithms for different healthcare applications is gaining interest at a steady pace. However, use of such algorithms can prove to be challenging as they require large amounts of training data that capture different possible variations. This makes it difficult to use them in a clinical setting since in most health applications researchers often have to work with limited data. Less data can cause the deep learning model to over-fit. In this paper, we ask how can we use data from a different environment, different use-case, with widely differing data distributions. We exemplify this use case by using single-sensor accelerometer data from healthy subjects performing activities of daily living - ADLs (source dataset), to extract features relevant to multi-sensor accelerometer gait data (target dataset) for Parkinson's disease classification. We train the pre-trained model using the source dataset and use it as a feature extractor. We show that the features extracted for the target dataset can be used to train an effective classification model. Our pre-trained source model consists of a convolutional autoencoder, and the target classification model is a simple multi-layer perceptron model. We explore two different pre-trained source models, trained using different activity groups, and analyze the influence the choice of pre-trained model has over the task of Parkinson's disease classification.

==> 07_References.tex <==
\vspace{-0.05in}
\section{References}\label{references}
\vspace{-0.05in}

[1] Anirudh Attractor Shape Descriptors
\newline [2] Anirudh Multi-Scale Attractor Shape Descriptors
\newline [3] Anirudh PI-Net Paper
\newline [4] Short Survey of Topological Data Analysis
\newline [5] Persistence Based Structural Recognition
\newline [6] Short Survey of Topological Data Analysis in Time Series and Signals Analysis
\newline [7] Perturbation Robust Representations of \newline Topological Persistence Diagrams
\newline [8] World Health Organization, Neurological Disorders Public Health Challenges (2006). June 2018
\newline [9] Paper with Statistics on Prevalence of PD
\newline [10] A survey of Parkinson's disease patients: most bothersome symptoms and coping preferences.
\newline [11] Deterioration of Parkinson’s disease during hospitalization: survey of 684 patients (Canada?)
\newline [12] A Step Towards the Automated Diagnosis of Parkinson’s Disease: Analyzing Handwriting Movements
\newline [13] Fully Automated Assessment of the Severity of Parkinson’s Disease from Speech
\newline [14] A deep learning approach for Parkinson’s disease diagnosis from EEG signals
\newline [15] Automatic recognition of gait-related health problems in the elderly using machine learning
\newline [16] Machine learning on brain MRI data for differential diagnosis of Parkinson’s disease and Progressive Supranuclear Palsy
\newline [17] Persistence Images: A Stable Vector Representation of Persistent Homology
\newline [18] Mathematical Tools for Shape Analysis and Description
\newline [19] Machine learning for Medical Diagnoses: history, state of the art and perspective
